Fast Stochastic Composite Minimization and an Accelerated Frank-Wolfe Algorithm under Parallelization

We consider the problem of minimizing the sum of two convex functions. One of those functions has Lipschitz-continuous gradients, and can be accessed via stochastic oracles, whereas the other is "simple". We provide a Bregman-type algorithm with accelerated convergence in function values to a ball containing the minimum. The radius of this ball depends on problem-dependent constants, including the variance of the stochastic oracle. We further show that this algorithmic setup naturally leads to a variant of Frank-Wolfe achieving acceleration under parallelization. More precisely, when minimizing a smooth convex function on a bounded domain, we show that one can achieve an $\epsilon$ primal-dual gap (in expectation) in $\tilde{O}(1/ \sqrt{\epsilon})$ iterations, by only accessing gradients of the original function and a linear maximization oracle with $O(1/\sqrt{\epsilon})$ computing units in parallel. We illustrate this fast convergence on synthetic numerical experiments.

==> motivation.tex <==
\section{Motivation}
\subsection{Overview of AGD+}
AGD+ \cite{diakonikolas2021complementary} focuses on problems of the of the form
\begin{align}
    \min_{y} F(y) := \G(y) + \h(y)
\end{align}
\begin{assumption}
\label{assumption:acc-breg-smooth-sc}
The function $G$ is convex and $\Lg$-smooth and the function $H$ is $\muh$-strongly convex.
\end{assumption}
The algorithm consists of three iterates $(z_k, y_k, v_k)$ and an increasing scalar sequence $\{A_k\}$. The algorithm requires a strongly-convex distance-generating function $w$. The updates read
\begin{align}
    \tau_k &= 1- A_k / A_{k+1}\\
    v_k &= (1 - \tau_k) y_k + \tau_k z_k\\
    \label{AGD:update}
    d_{k+1} &= d_k + (A_{k+1} - A_k) \nabla \G(v_k)\\
    z_{k+1} &\in \argmin\left\{ \inner{d_{k+1}}{y} + A_{k+1} \h(y) + \Lg \w(y)\right\}\\
    y_{k+1} &= (1 - \tau_k)y_k + \tau_k z_{k+1}
\end{align}
If $y^* \in \argmin F$, results from \cite{diakonikolas2021complementary} imply that
\begin{align*}
    F(y_k) - F(y^*) \leq O\left(\exp\left( -k \sqrt{\frac{\muh}{\Lg}}\right) \Lg D_\w(z_0, y^*)\right)
\end{align*}

For a convex compact set $K \subset \R^n$, we are interested in solving
\begin{align}
    \min_{x \in \R^n} f(x) + I_K(x)
\end{align}
where $f$ is convex and $L$-smooth. The Fenchel dual reads
\begin{align}
    \min_{y \in \R^n}  f^*(y) + \sigma(-y)
\end{align}
The first term $f^*$ is $1/L$-strongly convex, but the second term $\sigma$ is not smooth. Instead we smooth it using the aforementioned perturbed oracle and study the problem
\begin{align}
    \min_{y \in \R^n}  f^*(y) + \sigma_\epsilon(-y)
\end{align}
where $\sigma_\epsilon$ is $\frac{1}{\epsilon}$-smooth. As mentioned above, the convergence rate of AGD+ for such a problem is $O\left(\exp\left( - k \sqrt{\frac{\epsilon}{L}}\right)\right)$. However it requires computation of $\nabla \sigma_\epsilon$, which as discussed above cannot be computed exactly. However, by sampling from the distribution $\Delta$, we can computer a stochastic gradient. The question is whether we can replace $\nabla G(v_k)$ by a stochastic gradient in equation (\ref{AGD:update}). If the stochastic gradients have variance $\sigma^2$, one can expect a rate for stochastic AGD+ of the form
\begin{align}
    \exp\left( - k \sqrt{\frac{\muh}{\Lg}}\right) + \frac{\sigma^2}{\sqrt{\muh\Lg}}.
\end{align}
Indeed, the dependence of the form $\nicefrac{1}{\sqrt{\muh\Lg}}$ on the noise is typical of accelerated stochastic first order methods (need citation).
